Toyteller: AI-powered Visual Storytelling Through Toy-Playing with Character Symbols

We introduce Toyteller, an AI-powered storytelling system where users generate a mix of story text and visuals by directly manipulating character symbols like they are toy-playing. Anthropomorphized symbol motions can convey rich and nuanced social interactions; Toyteller leverages these motions (1) to let users steer story text generation and (2) as a visual output format that accompanies story text. We enabled motion-steered text generation and text-steered motion generation by mapping motions and text onto a shared semantic space so that large language models and motion generation models can use it as a translational layer. Technical evaluations showed that Toyteller outperforms a competitive baseline, GPT-4o. Our user study identified that toy-playing helps express intentions difficult to verbalize. However, only motions could not express all user intentions, suggesting combining it with other modalities like language. We discuss the design space of toy-playing interactions and implications for technical HCI research on human-AI interaction.

==> sections/00_teaser.tex <==

  \includegraphics[width=\textwidth]{figures/toyplaying-teaser.pdf}
  \caption{Interactions in \sys{}. a) \sys{} enables visual storytelling with AI through \textit{toy-playing} interaction with character symbols that accompany story texts. These character symbols can become both 1) a means to express the user's intention about the story unfolding and 2) a generation target that will be a part of the final visual story. For example, given a story setting defined as open-ended text, the user can physically manipulate symbols representing two story characters, and \sys{} can generate a story sentence that aligns with the user-provided character motions. b) \sys{} allows users flexibility in deciding which part of the output artifact (symbol motions, story texts) is created by the user or by the AI.}
  %\Description{On the left, there is a subfigure titled "Toy-playing-based AI-powered Storytelling." Under that, there is "Story setting" with two characters. Each character has a portrait in a triangular shape. The first character is "Amelia Harrington. 28. Independent and headstrong, constantly pushing boundaries. Her curiosity about the distorted sky may lead her into conflicts with authority figures or those trying to maintain order." The second character is "Ethan Blackwell. 35. A seasoned government agent tasked with containing knowledge of the distorted sky, putting him at odds with Amelia's inquisitive nature. His rigid adherence to protocols could create friction as he seeks to maintain secrecy and control over the situation." Below it, there is a description of a scene, "Amelia and Ethan ran into each other in a market." There is a figure with a name "An example toy-playing interaction," where the user is manipulating character symbols by making them move, and the AI is telling a following story sentence: "Ethan Blackwell followed Amelia Harrington as she slipped through the crowded market, his eyes locked onto the determined set of her shoulders." On the right, there is a subfigure with a name "Flexibility in Dividing Roles in Toy-playing-based AI-powered Storytelling." There are two parts in this subfigure, with the first part dividing roles between AI as "(Human/AI) manipulates all character symbols" and "(AI/Human) creates story texts." The second part is saying "(Human/AI) manipulates a part of character symbols" and "(AI/Human) manipulates a part of character symbols and creates story texts.}
  \label{fig:teaser}
